SDFReg: Learning Signed Distance Functions for Point Cloud Registration

Learning-based point cloud registration methods can handle clean point clouds well, while it is still challenging to generalize to noisy, partial, and density-varying point clouds. To this end, we propose a novel point cloud registration framework for these imperfect point clouds. By introducing a neural implicit representation, we replace the problem of rigid registration between point clouds with a registration problem between the point cloud and the neural implicit function. We then propose to alternately optimize the implicit function and the registration between the implicit function and point cloud. In this way, point cloud registration can be performed in a coarse-to-fine manner. By fully capitalizing on the capabilities of the neural implicit function without computing point correspondences, our method showcases remarkable robustness in the face of challenges such as noise, incompleteness, and density changes of point clouds.

==> src/2-relatedwork.tex <==
\section{Related Work}

\subsection{Point Cloud Registration}

\noindent\textbf{Correspondence-based Methods.} Correspondence-based registration methods calculate pose transformation by collecting corresponding points between two point clouds, including optimization-based and deep learning-based methods. The optimization-based works\cite{ICP,NDT,PLICP,LM-ICP,broad} typically minimize geometric projection errors through two stages: iterative correspondence search and pose estimation by an SVD solver. Deep learning-based methods\cite{Ppfnet,DCP,DeepGMR,prnet,GTFR,3D-3D,accelerating,registration} introduce deep neural networks to learn the correspondence points. Then, they compute the transformation matrix using SVD\cite{svd} or RANSAC\cite{ransac}, which is a one-step process that does not require iterating between correspondence estimation and transformation estimation. It should be noted that the correspondence search is affected by outliers and partial visibility in the point cloud, making the overall scheme less robust.

\noindent\textbf{Direct Registration Methods.} Direct registration methods omit the correspondence stage. 
Some traditional methods \cite{correspondencefree,richer} describe the point clouds with the implicit representation and optimize the distance error to obtain the registration parameters. However, these methods are limited by their model-fitting ability and generalization.
In addition, other learning-based methods\cite{PointNetLK,FMR,OMNet,REGTR,vrnet} estimate the transformation using neural networks in an end-to-end manner. Different from the methods based on correspondence search, these methods usually learn a pose-sensitive feature in a 
Euclidean space to represent the current pose. By aligning the features, the pose transformation can be predicted. However, since the methods learn from discrete point cloud samples, they are sensitive to noise and density changes.

%-------------------------------------------------------
\subsection{Learning Implicit Surface Representations}

Implicit neural representation recently gained a lot of attention, which is the backbone of many works on surface reconstruction and view synthesis. This representation directly learns the mapping between spatial coordinates and scene attributes, providing a fully differentiable and space-efficient way to represent 3D geometry. Occupancy and signed distance function (SDF) are two implicit surface representations. IM-Net~\cite{IM-Net} takes a coordinate as input and predicts a continuous value that represents the occupancy probability. This continuous value lies in the range [0, 1], where a value of 0 indicates empty space and a value of 1 indicates occupied space.  DeepSDF~\cite{deepsdf} implicitly models the distance from the query location to the closest point on the surface of the shape using deep neural networks. The SDFs are negative inside the shape, positive outside, and zero on the surface. The other representative works of implicit neural representation are OccNet\cite{OccNet}, ConvOccNet\cite{Conv_occupancy}, SAL\cite{Ini_Sdf}, VolSDF\cite{volsdf}, NeRF\cite{NeRF}, NeuS\cite{NeuS}, HF-NeuS\cite{hfneus} and GenSDF\cite{GenSDF}. Among these works, GenSDF proposes a semi-supervised meta-learning method that exploits the geometric relationship between labeled and unlabeled data of non-overlapping categories to train neural networks for implicit surfaces.

Implicit surfaces model a shape continuously, up to the infinite resolution. The methods such as\cite{ndf, deepsdf, neural, learningsdf, implicit} can smooth the noise of point clouds and complete the missing parts. These methods provide an opportunity for registration to avoid the effects of noise, outliers, and density changes in the point cloud. In this work, we propose a novel point cloud registration framework that leverages learnable implicit surfaces for point cloud registration, which is robust to point density change, noise, and missing data.

